Massive Stellar Triples Leading to Sequential Binary Black-Hole Mergers in the Field

Stellar triples with massive stellar components are common, and can lead to sequential binary black-hole mergers. Here, we outline the evolution towards these sequential mergers, and explore these events in the context of gravitational-wave astronomy and the pair-instability mass gap. We find that binary black-hole mergers in the pair-instability mass gap can be of triple origin and therefore are not exclusively formed in dense dynamical environments. We discuss the sequential merger scenario in the context of the most massive gravitational-wave sources detected to date: GW170729 and GW190521. We propose that the progenitor of GW170729 is a low-metallicity field triple. We support the premise that GW190521 could not have been formed in the field. We conclude that triple stellar evolution is fundamental in the understanding of gravitational-wave sources, and likely, other energetic transientsas well.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
